Robust Tiny Object Detection in Aerial Images amidst Label Noise

Precise detection of tiny objects in remote sensing imagery remains a significant challenge due to their limited visual information and frequent occurrence within scenes. This challenge is further exacerbated by the practical burden and inherent errors associated with manual annotation: annotating tiny objects is laborious and prone to errors (i.e., label noise). Training detectors for such objects using noisy labels often leads to suboptimal performance, with networks tending to overfit on noisy labels. In this study, we address the intricate issue of tiny object detection under noisy label supervision. We systematically investigate the impact of various types of noise on network training, revealing the vulnerability of object detectors to class shifts and inaccurate bounding boxes for tiny objects. To mitigate these challenges, we propose a DeNoising Tiny Object Detector (DN-TOD), which incorporates a Class-aware Label Correction (CLC) scheme to address class shifts and a Trend-guided Learning Strategy (TLS) to handle bounding box noise. CLC mitigates inaccurate class supervision by identifying and filtering out class-shifted positive samples, while TLS reduces noisy box-induced erroneous supervision through sample reweighting and bounding box regeneration. Additionally, Our method can be seamlessly integrated into both one-stage and two-stage object detection pipelines. Comprehensive experiments conducted on synthetic (i.e., noisy AI-TOD-v2.0 and DOTA-v2.0) and real-world (i.e., AI-TOD) noisy datasets demonstrate the robustness of DN-TOD under various types of label noise. Notably, when applied to the strong baseline RFLA, DN-TOD exhibits a noteworthy performance improvement of 4.9 points under 40% mixed noise. Datasets, codes, and models will be made publicly available.

==> CLC.tex <==
\begin{algorithm}[t]
  \SetAlgoLined
  % \KwData{}
  % \KwResult{how to write algorithm with \LaTeX2e }
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{&positive samples set $\textbf{\textit{pos}}$ of size $N$, \\ 
  & classification scores $\textbf{\textit{cls}}$ of size $N \times C$, \\
  & ground truth labels $\textbf{\textit{gt\_labels}}$ of size $N$, \\ 
  & dynamic queue $\textbf{\textit{DQ}}$ of size $C \times C \times T$}
  \Output{&noisy samples set $\textbf{\textit{noisy}}$, \\ 
  & clean samples set $\textbf{\textit{clean}}$, \\ 
  & corrective ground truth labels $\textbf{\textit{new gt\_labels}}$}
  \BlankLine
  \emph{compute the $\textbf{\textit{DT\!M}}$ using the $\textbf{\textit{DQ}}$ and Eq.~\ref{con:DTM}}\;
  \For{$i \leftarrow 0$ \KwTo $N$}{
    $gt_i$ $\gets$ $ gt\_labels[i]$\; 
    $gt\_scores$ $\gets$ cls[$i$,$gt_i$]\; 
    % $scores_i$ $\gets$ cls[$i$,:]\;
    $scores_i,classes_i$ $\gets$ sorted($cls[i,:]$)\;
    \emph{ //ranked from height to low}\\
    \For{$j \leftarrow 0$ \KwTo $len(scores_i)$}{
        \lIf{$scores_{ij}$ $!=$ $gt\_scores$}
            {
            \\ \quad suspected class set $\gets$ $scores_i$[j]\;
            \\ \quad index $\gets$ $classes_i$[j]}
        \lElse{break}
    }
%     \If{suspected class set is empty}{
%         clean \gets $pos_i$\;
%     }
%     \If{suspected class set is not empty}{
% \For{$k \leftarrow 0$ \KwTo len(suspected class set)}
%         {
%             temp \gets suspected class set[k]$\;$
%             \lIf{temp $\geq$ DTM[index[k],index[k]]}
%             {
%                 \\ \quad  candidate class set \gets temp
%             }
%         }
%     }
    \eIf{suspected class set is empty}{
      clean $\gets$ $pos_i$\;
      new gt\_labels $\gets$ $gt_i$\;
      }{
      \For{$k \leftarrow 0$ \KwTo len(suspected class set)}
        {
            temp $\gets$ suspected class set[k]\;
            \lIf{&temp $\geq$ DTM[index[k],index[k]] and \\
             & \quad temp $\geq$ DTM[$gt_i$,index[k]]}
            {
                \\ \quad  candidate class set $\gets$ temp\;
                \\ \quad  candidate index $\gets$ index[k]}
        }
        \eIf{candidate class set is empty}{
            clean $\gets$ $pos_i$\;
            new gt\_labels $\gets$ $gt_i$\;
        }{
            noisy $\gets$ $pos_i$\;
            new gt\_labels $\gets$ candidate index[0]\;
            
        }
    }
    }
      \label{on:CLC} 
  \caption{The proposed CLC method}
\end{algorithm}
